RiEMann: Near Real-Time SE(3)-Equivariant Robot Manipulation without Point Cloud Segmentation

We present RiEMann, an end-to-end near Real-time SE(3)-Equivariant Robot Manipulation imitation learning framework from scene point cloud input. Compared to previous methods that rely on descriptor field matching, RiEMann directly predicts the target poses of objects for manipulation without any object segmentation. RiEMann learns a manipulation task from scratch with 5 to 10 demonstrations, generalizes to unseen SE(3) transformations and instances of target objects, resists visual interference of distracting objects, and follows the near real-time pose change of the target object. The scalable action space of RiEMann facilitates the addition of custom equivariant actions such as the direction of turning the faucet, which makes articulated object manipulation possible for RiEMann. In simulation and real-world 6-DOF robot manipulation experiments, we test RiEMann on 5 categories of manipulation tasks with a total of 25 variants and show that RiEMann outperforms baselines in both task success rates and SE(3) geodesic distance errors on predicted poses (reduced by 68.6%), and achieves a 5.4 frames per second (FPS) network inference speed. Code and video results are available at https://riemann-web.github.io/.

==> sections/rebuttal.tex <==
\section{General Response to All Reviewers}

We thank all reviewers for the time and effort you have dedicated to reviewing our paper. We greatly appreciate your insightful comments and questions. In this section, we address some common concerns, and in the following sections, we address each reviewer's problems individually. We hope this response could answer your questions and clear your concerns. We have updated our paper and supplementary materials, with the changed parts highlighted in \textcolor{blue}{blue} color.

\subsection{Emphasis on The Novelty}
\label{novelty}

We notice that some reviewers pay too much attention to the network designing part (the saliency map network and the position-orientation network), and omit the problem formulation part stated in Section 3 of our paper. We apologize for previous unclear and misleading aspects of our original paper. We re-organize the introduction section and clearly state three main contributions of our paper at the end. Here we re-emphasize the novelty of our paper:
\begin{itemize}
    \item We propose the first end-to-end SE(3)-equivariant visuomotor policy learning framework for 6-DOF manipulation tasks by our specially designed SE(3)-equivariant action space. The end-to-end framework has potential for future large-scale training for diverse SE(3)-equivariant manipulation tasks;
    \item We design a saliency map network together with position and orientation networks as the policy model to achieve efficient SE(3)-equivariant training and near real-time inference speed (5.4 FPS);
    \item We achieve state-of-the-art success rates and pose estimation accuracy (reducing the SE(3)-geodesic distance error by 68.6\%) on a set of pick-and-place tasks under various settings, and we are the first to perform SE(3)-equivariant articulated object manipulation tasks through end-to-end training.
\end{itemize}

\subsection{Other Common Concerns}
\label{common}

\textcolor{blue}{Q1: Can we use pretrained object detection model or segmentation model to replace the saliency map module in \name?} (asked by the Area Chair wq6L and reviewer IVK7)

\textcolor{JungleGreen}{A1:} Firstly, the saliency map is a scene-level module, and using the scene-level module can support sequential pick-and-place tasks, which is what SAM or object detection modules cannot do, as demonstrated in D-EDFs~\cite{dedf}. For example, if the task is \textit{first pick up the blue cube onto the shelf, then pick up the JungleGreen cube onto the blue cube}, the saliency map module can predict different target objects at different time steps, but the object detection modules or SAM cannot do that. Note in this setting, we do not explicitly specify the object name. We want the robot to automatically learn the correct sequence from demonstrations.

Secondly, in practice, zero-shot 3D object detection or segmentation for any object is non-trivial and is still being actively studied by researchers~\cite{sam3ddet,sam3dseg,cen2023segment}, especially for cases with distracting objects. Meanwhile, the real-time performance will also be compromised (at least 2 seconds inference time for the current fastest 3D SAM method~\cite{cen2023segment}).

Finally, using SAM or object detection modules requires extra human semantic knowledge to specify ``which object is the target object", which is not contained in our demonstration.

Thus, we think we cannot use a pretrained object detection model or SAM to replace the saliency map in \name.

\textcolor{blue}{Q2: Why does \name\ use the SE(3)-geodesic distance as a metric? Is it a tailored metric for \name?} (asked by the Area Chair wq6L and reviewer IVK7)

\textcolor{JungleGreen}{A2:} As stated in the paper, we point out that although the success rate is a common metric for manipulation tasks, it is influenced by many elements. For example, if the size of the mug handle is larger, the \textit{mug-on-rack} task will become easier, which destroys the fairness of comparison. Thus for our SE(3)-equivariant problem, it is necessary to \textit{quantitatively} evaluate how well the SE(3)-equivariant feature is predicted. Here, we evaluate the SE(3)-geodesic distance between the ground truth target pose and the predicted ones. 

SE(3)-geodesic distance is a standard metric~\cite{bump2004lie} to evaluate the distance between two SE(3) group elements. It is \textit{not} a tailored metric for \name. We can also use Chordal distance, but we cannot directly use the Euclidean distance of two SE(3) pose matrices as the distance because it is not a legally defined distance: it is not rotational invariant (the Euclidean distance between two rotation matrices does not keep unchanged when they rotate).

\textcolor{blue}{Q3: Where does the generalization ability of \textit{new instance} or new geometry come from?} (asked by the Area Chair wq6L and reviewer EYRO)

\textcolor{JungleGreen}{A3:} The generalization ability of \name\ on the new geometry comes from the neural network structure and its inductive bias. We think it is the locality property of the message-passing mechanism in the equivariant backbone that brings this geometry-level generalization. We perform the \textit{new instance} experiments because, in related works~\cite{edf,dedf}, they found that equivariant networks have a certain degree of geometric generalization ability only with 5 to 10 demonstrations, and we confirmed this point in our experiments. Yes, compared to NDFs~\cite{ndf,rndf}, our geometry generalization ability is worse because their encoder is trained on a large-scale in-category dataset.

To better demonstrate how strong the generalization ability of \name\ is on new object geometries, here we add an additional experiment. We gradually deform the mesh of the mug trained in the \textit{mug-on-rack} task, put them into the \textbf{NP} setting, and record the corresponding SE(3)-geodesic error of the predictions from the original trained model. We keep the longest side of the mug the same. The results are in Table \ref{tab:geometry}.

\begin{table}[h]
\centering
\caption{SE(3)-geodesic distance evaluations of the trained model on the training mug. Each value is evaluated under 20 random SE(3) poses.}
\label{tab:geometry}
\begin{tabular}{c|c|c|c|c|c}
\toprule
Picture & \includegraphics[width=0.1\linewidth]{figures/original_mug.png} & \includegraphics[width=0.1\linewidth]{figures/mug_1.png} & \includegraphics[width=0.1\linewidth]{figures/mug_2.png} & \includegraphics[width=0.1\linewidth]{figures/mug_3.png} & \includegraphics[width=0.1\linewidth]{figures/mug_4.png} \\
Description & original & \makecell{flat} & \makecell{tall} & fat & new\\
\midrule
% 在此处插入图片
$\mathcal{D}_{geo}$ & 0.055 & 0.187 & 0.127 & 0.094 & 0.395\\
\bottomrule
\end{tabular}
\end{table}

We can see that if the general shape of the mug remains (especially for the rim of the mug), the $\mathcal{D}_{geo}$ remains at a low level, which shows that \name\ has a certain power of geometry generalization ability. However, if the geometry of the mug is deformed too much, the result becomes worse.

\section{Response to The Area Chair wq6L}

\textcolor{blue}{Q1: The introduction is too lengthy.}

\textcolor{JungleGreen}{A1:} Thanks for your suggestion. We have modified the introduction section, streamlined the description of related work and emphasized the contributions of \name. Please check our updated paper.

\textcolor{blue}{Q2: Lack of evidence of the claims in the introduction.}

\textcolor{JungleGreen}{A2:} Thanks for your questions. We apologize for the lack of rigor in our previous version. Here we give the detailed provenance of claims in the introduction section.

\begin{itemize}
    \item [1)] ``\textit{... the two-stage paradigm of NDFs~\cite{ndf} makes it hard to fine-tune on new object categories...}". This is a judgment made and illustrated by the EDF~\cite{edf} paper (stated in line 19). The meaning of this claim is that, because two-stage methods~\cite{ndf,rndf,equivact} use a pretrained encoder for a specific category of objects, their networks cannot be directly applied to a new object category with 5 to 10 demonstrations since they need to collect numerous new object data to retrain a new encoder. Instead, \name\ can be applied on any new object with 5 to 10 demonstrations since \name\ is a novel end-to-end SE(3)-equivariant manipulation framework.

    \item [2)] \textit{...still need to separate the robot end-effector and the grasped target object point cloud from the scene to perform the time-consuming (around 10s) descriptor field matching process for every inference}  This is from the experiment results of the related papers~\cite{ndf,rndf,edf,dedf}, to be specific, Section A.5.5 of~\cite{rndf}, Table 4 of~\cite{edf}, and Section E.2.2 of~\cite{dedf}.
\end{itemize}

\textcolor{blue}{Q3: Is the time-consuming matching process of~\cite{ndf,edf,rndf,dedf} an issue of unoptimized code or something that can be further improved by additional compute or is this a fundamental limit on the speed of the algorithm?}

\textcolor{JungleGreen}{A3:} It is a fundamental limit of the field-matching algorithms. This time-consuming period is for the energy-based optimization process (nothing to do with the neural networks).

A quicker optimization time (which usually means a smaller optimization step) usually causes the optimization to frequently fail to converge (see Section E.2.2 of~\cite{dedf}). Although some faster optimization methods (such as cooperative learning~\cite{xie2018cooperative,xie2021cooperative} and amortized sampling~\cite{xie2021learning,wang2016learning}) can be used here to accelerate this process, we believe this is non-trivial and the contribution of this exploring alone warrants another paper. 

\textcolor{blue}{Q4: How does one set up collision constraints without segmenting the scene? For example, I would have to know what set of the point cloud/environment is okay to touch and what is not.}

\textcolor{JungleGreen}{A4:} During the planning, we open the gripper of the robot, and every point of the point cloud is not touchable. The planner drives the end-effector to the target pose with collision avoidance, and after the end-effector reaches the target pose, we close the gripper to make contact with (or grasp) the target object.

The planner we used in this work is a point-cloud-based planner, implemented in MPlib~\cite{MPlib} with state-of-the-art sampling-based motion planning algorithms in OMPL. You may also check \href{https://sapien.ucsd.edu/docs/latest/tutorial/motion_planning/collision_avoidance.html}{this link} for a demo.

\textcolor{blue}{Q5: Can we use SAM to replace the saliency map module?}

\textcolor{JungleGreen}{A5:} Answered in \textcolor{JungleGreen}{A1} of Section~\ref{common}.

\textcolor{blue}{Q6: Lack of experiment results for the claim ``\textit{search and generative processes are slower and that a conditional approach with a simplistic inference procedure (forward passes of neural networks) should be adopted}".}

\textcolor{JungleGreen}{A6:} We apologize for the previous insufficiently rigorous claim. We have deleted this statement in the new version. 

For time comparison between \name\ and field matching methods, we refer to Table \ref{tab:time} and the real-time following demo in our video. For the comparison of the final results, we think the success rate is more like a ``qualitative" metric as stated in \textcolor{JungleGreen}{A2} in Section \ref{common}, thus similar success rates near 100\% cannot really reflect the effectiveness of different methods. We propose to ``quantitatively" evaluate them with SE(3)-geodesic distance (which only relies on the pose estimation performance), and we show that \name\ can greatly surpass baselines.

\textcolor{blue}{Q7: The SE(3)-geodesic distance metric is like a specific metric that the approach is tailored to work well against.}

\textcolor{JungleGreen}{A7:} Answered in \textcolor{JungleGreen}{A2} of Section~\ref{common}.

\textcolor{blue}{Q8: There has to be a more convincing case made on generalization across novel distributions of object geometry.}

\textcolor{JungleGreen}{A8:} Answered in \textcolor{JungleGreen}{A3} of section~\ref{common}.

\section{Response to Reviewer Lypd}

\textcolor{blue}{Q1: This paper would be greatly strengthened if the results section had more clearly identified claims that were well supported by their quantitative results.}

\textcolor{JungleGreen}{A1:} Thanks for your suggestion. We have updated the experiment section to better show our achievements.

\textcolor{blue}{Q2: Copyright of citing lecture notes~\cite{geodistance}.}

\textcolor{JungleGreen}{A2:} Thanks for your correction. We substitute this citation with a published material~\cite{bump2004lie}.

\textcolor{blue}{Q3: Does the acceleration of \name\ come from the code implementation?}

\textcolor{JungleGreen}{A3:} For the inference time, no. The reason why D-EDF~\cite{dedf} is slow is because of its optimization process, which does not correlate with the network implementation. In contrast, \name\ can directly predict actions with the network forward process.

For the training time, it is difficult to fairly compare different backbones in different algorithm frameworks, since the training time not only contains network forward time but also other times such as the optimization process in D-EDF~\cite{dedf}. However, the training time of \name\ is not the main contribution of this paper. We just want to show that \name\ can be trained in a similar time compared to current SOTA methods.

\textcolor{blue}{Q4: The authors very confusingly claim that EDF and “D-EDF achieve “similar results” for the reported metrics but are inferior approaches due to undesirable characteristics of the methods (i.e. field matching reliance and not producing needed physical quantities) which result in \name\ achieving the best performance.}

\textcolor{JungleGreen}{A4:} We apologize for the confusing statement. We have updated the corresponding experiment section and replaced these confusing statements with rigorous ones. Here we originally mean two things: 1) the baseline methods are worse than \name\ according to Table 1 and Table 2; 2) the baseline methods cannot predict physical quantities (the directional action) for the \textit{open-faucet} task.

\textcolor{blue}{Q5: What are the ``training and testing settings" in the experiments?}

\textcolor{JungleGreen}{A5:} We apologize for the confusing term. We have updated the corresponding section. Here our original meaning is that, the ``training setting" and ``testing setting" are all test settings, and the ``training setting" means \textbf{T}, where the experiments are tested on the same configurations as training but with different random seeds. For example, the area of the mug is the same quarter of the table, but the specific location of the mug is randomized for each episode. And the ``testing setting" means \textbf{NI}, \textbf{NP}, \textbf{DO}, and \textbf{ALL}.

\section{Response to the Reviewer EYro}
\label{EYro}

\textcolor{blue}{Q1: Can authors show examples of \name\ on low quality point clouds?}

\textcolor{JungleGreen}{A1:} Sure. In fact, in our real-world experiment, a considerable part of the data is of low quality. We do not assume the real-world object point clouds are intact, so all of the real-world experiments are in the same relatively low quality. Here we show some examples in Figure \ref{fig:data_quality}:

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/rebuttal_partial1.png}
        \caption{Pose and heatmap prediction of the \textbf{NP} test setting of \textit{mug-on-rack}. A significant part of the point cloud is  missing.}
        \label{fig:mug_rebuttal}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/rebuttal_partial2.png}
        \caption{Pose and heatmap prediction of the \textbf{DO} test setting of \textit{mug-on-rack}. A noisy part (opposite of the handle) is on the mug.}
        \label{fig:plane_rebuttal}
    \end{subfigure}
    \caption{Visualization of the low-quality data in the real-world experiments. \name\ can still give good predictions under such circumstances.}
    \label{fig:data_quality}
\end{figure}

In practice, it is difficult for only 4 fixed cameras in the real world to capture such a whole scene, and thus all real-world data are of lower quality than the simulation. This is the reason why the results in Table \ref{tab:real-world} are worse than the results in the simulation. Such low-quality data can compromise the integrity of the object geometric information.

\textcolor{blue}{Q2: \name\ cannot model the multi-modality in the data, so \name\ struggles with symmetric objects, which is supported by other methods for rearrangement that utilize continuous optimization and/or de-noising diffusion.}

\textcolor{JungleGreen}{A2:} Theoretically, we point out that if the object is symmetrical and the demonstrations are multi-modal (grasping different parts of the same object), the SE(3)-equivariance will \textit{conflict} with the multi-modal data, because we cannot tell the SE(3) configuration of the object since it is symmetrical. Consider the example of \textit{pick-up-bowl}: the bowl is symmetrical along the vertical axis. If actions of picking the edge of the bowl in different positions are demonstrated, there will be confusion when the bowl is in a different configuration, as shown in Figure \ref{fig:bowl}. We can either say \textit{the bowl looks the same as previous ones, so we do the same}, or we can say \textit{the bowl is rotated by 180$^{\circ}$, so we also rotate the action by 180$^{\circ}$}. Both of them are correct solutions.

\begin{figure}[h]
    \centering
        \includegraphics[width=0.49\textwidth]{figures/rebuttal_bowl.png}
    \caption{Visualization of the symmetry problem.}
    \label{fig:bowl}
\end{figure}

If the object is not symmetrical, and there are multi-modality demonstrations, our MSE loss is theoretically inferior to the denoising diffusion loss. However, in the D-EDF~\cite{dedf} paper, they do not show any multi-modality experiments, nor in other related papers~\cite{ndf,edf,rndf,equivact}. Therefore, we can say that SE(3)-equivariant manipulation with multi-modal demonstrations remains an unexplored problem.

\textcolor{blue}{Q3: Do the objects used for placing/hanging change shape or pose?}

\textcolor{JungleGreen}{A3:} They do change pose. However, they do not change shape, because \name\ only has limited geometry generalization ability, as answered in the \textcolor{JungleGreen}{A3} in Section \ref{common}.

\textcolor{blue}{Q4: Does it ever have problems predicting certain translations, such as placing poses that are far from any visible points?}

\textcolor{JungleGreen}{A4:} Thanks for your detailed observation. In fact, we introduce a translation offset (only one for all demonstrations of the same object) for the hanging action, and the robot will add this offset to the predicted target pose during execution. This can support cases where the target pose is not in the convex hull of the point cloud of the object. We have added these details in the updated version of the script.


\begin{table*}[h]
\centering
\caption{Success rates and SE(3)-geodesic distances of different $r_1$ and $r_2$ of the \textit{mug-on-rack} task in simulation. Each value is evaluated under 20 random seeds. In our original paper, we choose $r_1=0.16m$ and $r_2=0.02m$.}
\label{tab:success_rate_r1r2}
% 使用S列类型来对齐小数点
\sisetup{table-format=1.2} % 设置数字的格式，这里是最多一个小数位
\begin{tabular}{
  l
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
}
\toprule
\multicolumn{2}{c}{$r_1/m$} & \multicolumn{3}{c}{$0.05$} &
\multicolumn{3}{c}{$0.10$} &
\multicolumn{3}{c}{\makecell{$0.16$}} &
\multicolumn{3}{c}{\makecell{$0.22$}} &
\multicolumn{3}{c}{\makecell{$0.28$}} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
\cmidrule(lr){12-14}
\cmidrule(lr){15-17}
\multicolumn{2}{c}{$r_2/m$} & 0.01 & 0.02 & 0.04 & 0.01 & 0.02 & 0.04 & 0.01 & 0.02 & 0.04 & 0.01 & 0.02 & 0.04 & 0.01 & 0.02 & 0.04 \\
\midrule
 & \textbf{T} & 0.00 & 0.00 &  0.00 & 0.50 & 0.85 & 0.80 & 0.90 & \cellcolor{cellbgcolor} 1.00 & \cellcolor{cellbgcolor} 1.00 & 0.90 & \cellcolor{cellbgcolor} 1.00 & \cellcolor{cellbgcolor} 1.00 & 0.95 & \cellcolor{cellbgcolor} 1.00 & \cellcolor{cellbgcolor} 1.00 \\
 & \textbf{NI} & 0.00 & 0.00 &  0.00 & 0.10 & 0.80 & 0.75 & 0.80 & 0.90 & \cellcolor{cellbgcolor} 0.95 & 0.90 & \cellcolor{cellbgcolor} 0.95 & 0.90 & 0.90 & 0.90 & \cellcolor{cellbgcolor} 0.95 \\
SR & \textbf{NP} & 0.00 & 0.00 &  0.00 & 0.45 & 0.75 & 0.80 & 0.85 & 0.95 & \cellcolor{cellbgcolor} 1.00 & 0.90 & 0.95 & 0.95 & 0.95 & 0.95 & \cellcolor{cellbgcolor} 1.00 \\
  & \textbf{DO} & 0.00 & 0.00 &  0.00 & 0.35 & 0.80 & 0.70 & 0.70 & \cellcolor{cellbgcolor} 1.00 & \cellcolor{cellbgcolor} 1.00 & 0.85 & 0.95 & \cellcolor{cellbgcolor} 1.00 & 0.80 & \cellcolor{cellbgcolor} 1.00 & \cellcolor{cellbgcolor} 1.00 \\
 & \textbf{ALL} & 0.00 & 0.00 &  0.00 & 0.00 & 0.50 & 0.55 & 0.50 & 0.85 & 0.85 & 0.70 & 0.85 & \cellcolor{cellbgcolor} 0.90 & 0.70 & 0.85 & 0.80 \\
\midrule
 & \textbf{T} & 1.366 & 1.478 & 1.175 & 0.688 & 0.178 & 0.186 & 0.278 & \cellcolor{cellbgcolor} 0.053 & 0.056 & 0.067 & 0.064 & 0.062 & 0.059 & 0.060 & 0.055 \\
 & \textbf{NI} & 1.159 & 1.759 & 1.311 & 0.982 & 0.220 & 0.201 & 0.321 & 0.066 & \cellcolor{cellbgcolor} 0.061 & 0.068 & \cellcolor{cellbgcolor} 0.061 & 0.062 & 0.066 & 0.063 & 0.062 \\
$\mathcal{D}_{geo}$ & \textbf{NP} & 1.668 & 1.076 & 1.079  & 0.804 & 0.123 & 0.202 & 0.339 & 0.069 & 0.066 & 0.063 & 0.066 & \cellcolor{cellbgcolor} 0.055 & 0.060 & 0.064 & 0.058 \\
 & \textbf{DO} & 1.460 & 1.298 & 1.290  & 0.866 & 0.175 & 0.199 & 0.297 & 0.058 & \cellcolor{cellbgcolor} 0.056 & 0.082 & 0.062 & 0.059 & 0.079 & 0.064 & 0.063 \\
 & \textbf{ALL} & 1.982 & 1.333 & 1.077  & 1.390 & 0.797 & 0.639 & 0.427 & 0.071 & 0.070 & 0.079 & 0.077 & \cellcolor{cellbgcolor} 0.068 & 0.088 & 0.079 & 0.072 \\
\bottomrule
\end{tabular}
\end{table*}


\textcolor{blue}{Q5: Were any sensitivity experiments done to understand the impact of the two radii values that are used in the saliency map and the orientation prediction? As I understand these are just hyperparameters of the method - was it difficult to obtain good values for these hyperparameters?}

\textcolor{JungleGreen}{A5:} Thanks for your question. Here we add additional experiments to answer this question. We train the \textit{mug-on-rack} task in the simulation with different $r_1$ and $r_2$. Results are in Table \ref{tab:success_rate_r1r2}.

Note in our paper, we choose $r_1=0.16m$ and $r_2=0.02m$. In the \textit{mug-on-rack} task, the height of the mug is about $0.22m$ and the width of the mug is about $0.20m$. Note $r_2=0.01m$ means that there is only one point for $\psi_2$ to perform mean pooling, because we perform point cloud voxelization for the point cloud with a voxel size of $0.01m$.

From the results, we can see that:
\begin{itemize}
    \item $r_1$ should be large enough ($\geq 0.16m$) to capture all points of the target objects to make sure the position and orientation network can understand the full object geometry. If $r_1$ is less than the radius of the mug, the success rate will drop quickly, and the SE(3) geodesic error will increase quickly. If $r_1$ is too small ($r_1=0.05m$), the success rate becomes zero. The reason is that the training becomes very unstable because every time the position and the orientation network may choose different parts of the point cloud for training since the saliency map network is not that strong to give very precise position predictions.

    \item $r_2$ should capture more than one point ($>0.01m$) to avoid noisy and accidental errors caused by too few points.

    \item Although $r_2=0.04m$ also works well, it brings more burden for training since the orientation network $\psi_2$ outputs the highest type-$l$ vectors in our whole pipeline, and using fewer points for training is better for reducing the memory usage for $\psi_2$.

    \item For $r_2=0.01m$, the results are significantly worse than other situations in \textbf{DO} and \textbf{ALL}. This shows that noisy points will influence the results if we only use one point for prediction.

    \item The worst SE(3)-geodesic error of \name\ ($r_1=0.05m$) is smaller than the R-NDF baseline~\cite{rndf} in Table \ref{tab:gdistance}. This is because the saliency map network will restrict the position error to be in a certain range.
\end{itemize}






\textcolor{blue}{Q6: Can the author elaborate more on the \textit{open-faucet} task?}

\textcolor{JungleGreen}{A6:} Sure. We add additional explanations in Section 4.3. Here we also give some explanations. 

For the \textit{open-faucet} task, we assume that given a target pose $\mathbf{T} = \{\mathbf{R}, \mathbf{t}\} \in SE(3)$ and a target direction $\mathbf{d} \in \mathbb{R}^3$, the robot can accomplish the task by first going to the target pose $\mathbf{T}$ just as done in pick-and-place tasks, and then moving along the target direction $\mathbf{d}$ while keeping the orientation not changed, as illustrated in Figure \ref{fig:faucet}. To encode the extra directional action $\mathbf{d}$, we add another type-$1$ vector field on the orientation network $\psi_2$, that is: $\mathbf{f}_R=\bigoplus_{i=1}^{4}\mathbf{f}_1^i(x), x\in \mathbf{B}_{ROI}$. The final output directional action $\hat{\mathbf{d}}$ is also calculated through mean pooling on points in the radius $r_2$. Note the policy needs to continuously predict the output direction during the opening process, which shows that \name\ can capture the local SE(3)-equivariance of the handle part of the faucet.

In this task, we give demonstrations of not only the target pose $\mathbf{T}$, but also the opening direction $\mathbf{d}$ at the first frame. Here there exists two kinds of SE(3)-equivariance: the target pose should be equivariant to the pose of the faucet at the first frame, and the opening direction should be equivariant to the handle during the opening process, where the second equivariance requires both local-equivariance and the real-time performance. 

\textcolor{blue}{Q7: Add an experiment comparison or detailed comparison between \name and SE(3) data augmented version of TAX-Pose~\cite{taxpose}.}

\textcolor{JungleGreen}{A7:} Thanks for your question. We have cited TAX-Pose~\cite{taxpose} in our new version. We do not think it is necessary to add an experiment for TAX-Pose. Here are some explanations and comparisons:
\begin{itemize}
    \item Although TAX-Pose~\cite{taxpose} is not essentially an SE(3)-equivariant backbone, it already achieves SE(3)-invariant manipulation because it pretrains its encoder on the in-category object dataset with various SO(3) configurations, as stated in Appendix E.2 of their paper, so there is no ``SE(3)-data augmentation" for TAX-Pose.

    \item The difference between TAX-Pose~\cite{taxpose} and R-NDF~\cite{rndf} is that in TAX-Pose they use a different approach to replace the feature field matching process (the cross attention module and the differential SVD process). However, as shown in their experiment results, R-NDF performs better in the \textit{mug-on-rack} tasks under arbitrary initial poses (63\% success rate in TAX-Pose, 75\% success rate in R-NDF). Thus we do not think it is necessary to do extra experiments for TAX-Pose.

    \item The differences between \name\ and TAX-Pose~\cite{taxpose} are: 1) TAX-Pose requires well-segmented point clouds as input, while \name\ directly takes as input the scene point cloud; 2) TAX-Pose can only predict one SE(3) pose for pick-and-place tasks, while \name\ can predict equivariant directional action for articulated object manipulation tasks; 3) TAX-Pose requires in-category object data to pretrain the encoder, while \name\ designs an end-to-end visuomotor training pipeline.
\end{itemize}

\textcolor{blue}{Q8: Where is the generalization to new instances coming from?}

\textcolor{JungleGreen}{A8:} Answered in \textcolor{JungleGreen}{A3} of Section \ref{common}.

\textcolor{blue}{Q9: Since this now runs at 5hz, is there any need to only perform tasks/imitate demos with a single/pair of gripper poses? Can we represent and imitate more temporally dense trajectories with this technique?}

\textcolor{JungleGreen}{A9:} Thanks for your good question. Yes, trajectory-level equivariance is a very interesting direction. While real-time inference speed is necessary for trajectory-level equivariance, 
%it still requires other properties. In fact, it has not been fully studied on SE(3)-equivariant robot manipulation tasks because 
it is very hard to define an \textit{equivariant trajectory} with a single-step equivariant backbone. The network cannot be a single-step network (like \name), but has to give a trajectory prediction at each time step, like done in the Diffusion Policy~\cite{diffusionpolicy}. We believe this is an interesting future direction, but it is totally out of the scope of this paper.

\textcolor{blue}{Q10: Figure 6 and Figure 8 are a bit messy and difficult to understand. I would suggest exploring ways to improve their quality + clarity.}

\textcolor{JungleGreen}{A10:} Thanks very mush for your suggestion! We have updated Figure 6 and Figure 8 (it becomes Figure 10 now) to make it more clear for readers.

\textcolor{blue}{Q11: Can the authors elaborate on how the final placing pose prediction works?}

\textcolor{JungleGreen}{A11:} Answered in \textcolor{JungleGreen}{A4}.

\textcolor{blue}{Q12: Is there a reason the paper focuses on generalizing unseen instances for the grasped object but not the objects used for placing/hanging?}

\textcolor{JungleGreen}{A12:} Answered in \textcolor{JungleGreen}{A3}.

\textcolor{blue}{Q13: Most of the object rotations demonstrated in the results only seem to have a limited rotation angle. Is there any reason for this discrepancy in the level of OOD orientations the method can handle?}

\textcolor{JungleGreen}{A13:} We apologize for the confusing shown cases in the previous version. \name\ definitely can also handle fully sideways objects. Please check the demo we showed at the beginning of the video, where we show the full SE(3) predictions on the mug.

\textcolor{blue}{Q14: What is the difference between $\hat{t}$ and $x_{t_1}$ ? Are these both supervised with the same ground truth transform? And are they flipped in the figure shown in the paper vs. the video?}

\textcolor{JungleGreen}{A14:} Thanks for your question. $\hat{t}$ is the prediction of the position network and $x_{t_1}$ is the prediction of the saliency map. They are supervised with the same ground truth. And yes, they are flipped by mistake. We apologize for the mistake, and we have corrected this in the updated video.

\section{Response to the Reviewer iVK7}

We sincerely thank you for your helpful feedback. Here we give detailed responses to your questions. We hope these explanations address your concerns and enhance your understanding of our work.

\textcolor{blue}{Q1: Lack of novelty: this work appears to be a mere system integration of saliency map prediction and SE(3) pick-place planning.}

\textcolor{JungleGreen}{A1:} Thanks for your question. We apologize for the confusion caused by our way of writing. We re-emphasize our novelty in Section \ref{novelty}, and we re-write part of the introduction section. Please check them and we hope they can solve your concern. 

Here we give some extra explanations. Firstly, we emphasize that we are the first to \textit{define} an end-to-end local SE(3)-equivariant robot manipulation framework, which directly outputs the target action and avoids the field-matching steps required by most related works~\cite{ndf,rndf,edf,dedf,taxpose,fouriertransporter,sampleefficient}. Secondly, we believe it is non-trivial to design and implement such a framework, which needs efforts to handle the non-equivariance caused by common action space parameterization (Euler-angle/quaternion/axis-angle), the non-orthogonal output of the rotation network, and the exorbitant computational cost given by the equivariant backbone. We would like to emphasize that handling each of these challenges is a non-trivial process.
%We hope the reviewer can understand that each of these points is not easy.

\textcolor{blue}{Q2: The contribution of the saliency map is not convincing.}

\textcolor{JungleGreen}{A2:} Answered in \textcolor{JungleGreen}{A1} in Section \ref{common}.

\textcolor{blue}{Q3: Misleading R-NDF baseline: R-NDF's input should be a segmented object point cloud.}

\textcolor{JungleGreen}{A3:} Firstly, we apologize for not illustrating the detailed experiment settings of R-NDF~\cite{rndf} in our submitted manuscript. In our experiments, we in fact sent the predicted $\mathbf{B}_{ROI}$ segmentation to R-NDF~\cite{rndf} rather than the point cloud of the entire scene. More specifically, $\mathbf{B}_{ROI}$ is the prediction produced by the saliency network, which contains the target object points as well as its surrounding point clouds. 
In doing so, we make sure that the inputs of R-NDF~\cite{rndf} and our position and orientation networks are the same, making the comparison as fair as possible.

The reason why we choose R-NDF~\cite{rndf} as a baseline is to compare the methods using Vector Neurons~\cite{vn} (a mainstream option for a number of previous equivariant robot manipulation works~\cite{ndf,rndf,equivact}) with our method, to show that they cannot perform well on unsegmented point clouds, even with a small ball of point clouds around the target object.

Secondly, it is suggested to use a ``segmentation module + R-NDF" as a better baseline. We believe that if perfect object point cloud segmentations were given, R-NDF (and other capable baselines) would perform well because this is exactly the experiment settings in their paper. However, effective and robust instance segmentation on 3D point clouds (rather than 2D images) is itself a non-trivial problem~\cite{sam3ddet,sam3dseg,cen2023segment}, which is far beyond the focus of our paper. Thus, we think this baseline is not necessary. Please also check \textcolor{JungleGreen}{A1} in Section \ref{common} for more explanations about using SAM in our method.
% Thus the result of this baseline will depend entirely on the effectiveness of the 3D segmentation model, which is not the objective of this paper. 

\textcolor{blue}{Q4: The author should change D-EDF~\cite{dedf} baseline to the one with the least amount of ``inference" time, which is what the paper claims to be their contribution.}

\textcolor{JungleGreen}{A4:} We choose D-EDF~\cite{dedf} as our baseline for two reasons: 1) it is the state-of-the-art SE(3)-equivariant manipulation method that does not need segmentation and only needs a handful of demonstrations. 2) It has the fastest training time, and has comparable inference time compared to previous methods~\cite{ndf,edf,rndf}. The training time comparison in Table 3 just aims to show that \name\ can be trained within a similar time compared to current SOTA methods. The training time of \name\ is \textit{not} the main contribution of this paper. We focus on the inference time.

\textcolor{blue}{Q5: Keep the batch size constant when comparing the training time for an apples-to-apples comparison.}

\textcolor{JungleGreen}{A5:} We keep the maximum GPU memory usage the same for a fair comparison (48GB).

\textcolor{blue}{Q6: Is there anything special about the ``position and orientation net," which is the core part of SE(3)-equivariant manipulation? Assuming that segmentation is already solved, highlighting the effectiveness of the ``position and orientation net" will make this work more powerful.}

\textcolor{JungleGreen}{A6:} Thanks very much for your suggestion. In fact, the position and orientation networks are one of the main contributions of this paper. They are both SE(3)-equivariant backbones. Our design of the orientation network is the first time to regress 3 SE(3)-equivariant axes as the rotation matrix, and in practice we design radius mean pooling (the $r_2$) to make this paradigm really work on real manipulation tasks. In theory, we also prove that other rotation parameterization choices are not SE(3)-equivariant so they cannot be directly regressed. Please check \textcolor{JungleGreen}{A5} in Section \ref{EYro} for detailed results of choosing different $r_2$.


Please also refer to Section \ref{novelty} and \textcolor{JungleGreen}{A1} for an explanation of the function of these two networks. 

\textcolor{blue}{Q7: It seems more effective to mention the actual GPU memory usage given the dataset specification, rather than mentioning the maximum batch size.}

\textcolor{JungleGreen}{A7:} Sure. For a given point cloud of 8192 points, \name\ only uses about 11GB of GPU memory.

\textcolor{blue}{Q8: Typos and mistakes.

\textcolor{JungleGreen}{A8:} Thanks for your suggestions. We have corrected these typos and mistakes. Please check our new version of the paper.}

\textcolor{blue}{Q9: Why R-NDF~\cite{rndf} is a strong baseline?}

\textcolor{JungleGreen}{A9:} This is because it has the highest success rates in SE(3)-equivariant manipulation methods that require point cloud segmentation~\cite{ndf,rndf,equivact} (75\% on the \textit{mug-rack} task with arbitrary initial poses, reported in Figure 4 of their original paper). 

